Pairwise Margin Maximization for Deep Neural Networks

The weight decay regularization term is widely used during training to constrain expressivity, avoid overfitting, and improve generalization. Historically, this concept was borrowed from the SVM maximum margin principle and extended to multi-class deep networks. Carefully inspecting this principle reveals that it is not optimal for multi-class classification in general, and in particular when using deep neural networks. In this paper, we explain why this commonly used principle is not optimal and propose a new regularization scheme, called {\em Pairwise Margin Maximization} (PMM), which measures the minimal amount of displacement an instance should take until its predicted classification is switched. In deep neural networks, PMM can be implemented in the vector space before the network's output layer, i.e., in the deep feature space, where we add an additional normalization term to avoid convergence to a trivial solution. We demonstrate empirically a substantial improvement when training a deep neural network with PMM compared to the standard regularization terms.

==> 3_large_margin_DNN.tex <==
\section{Large Margin in DNNs}
\label{MMP_details}
Applying PMM directly to DNNs poses several problems. First, these networks employ a nonlinear mapping from the input space into a representation space: 
%$\phi_i= m(\x_i): {\cal X} \rightarrow {\Phi}$.  
$\phi_i= F(\x_i, \theta): {\cal X} \rightarrow {\Phi}$, where $\theta$ are the network parameters.  
The  vector $\phi_i$  can be interpreted as a feature vector based on which the last layer in a DNN calculates the scores for each class via a fully-connected layer,  $s_j(\phi_i)=\w_j^T \phi_i + b_j$. 
Maximizing the margin in the input space ${\cal X}$, as suggested in \cite{sokolic2017robust}, requires back-propagating derivatives along the network up to the input layer, and calculating distances to the boundary up to the first order approximation. In highly nonlinear mappings, this approximation becomes inaccurate very fast as we move away from the decision boundary. 
Therefore, we apply the large margin principle in the last layer, where the distances to the decision boundary are Euclidean in the feature space $\Phi$:
\begin{equation}
\label{eq:d3}
    d_{y_i,m_i}(\phi_i) =  \frac{\w_{y_i,m_i}^T \phi_i +b_{y_i,m_i}}{\| \w_{y_i,m_i} \|} 
\end{equation}

The second problem stems from the fact that in Equation~\ref{eq:d2}, the input space ${\cal X}$ is fixed along the course of training while the feature space $\Phi$ in Equation~\ref{eq:d3} is constantly changing. Accordingly, maximizing the margins in Equation \ref{eq:d3} can be trivially attained by scaling up the space $\Phi$.  Therefore, the feature space $\Phi$ must be constrained. In our scheme, we divide Equation \ref{eq:d3} by $\| \phi_{max}\|$, 
the maximal norm of the samples in the feature space, of the current batch.
%which is the sample with the maximal feature magnitude at the current batch. 
This ensures that scaling up the feature space will not increase the distance in a free manner. The proposed formulation is translated, similarly to Equation~\ref{eq:optim2}, into the following optimization problem 
\begin{equation}
\label{eq:d4}
\min_{W,\b}  \sum_i {\cal R}_i + \lambda \sum_i {\cal C}_i
\end{equation}
where 
$${\cal R}_i = \|\w_{y_i,m_i}\|^2 \|\phi_{max}\|^2 $$
denotes the margin regularization term, and ${\cal C}_i$ is the empirical risk term.
% \begin{equation}
% \label{eq:hinge}
% {\cal C}_i = \max (0, 1- (\w_{y_i,m_i}^T \phi_i + b_{y_i,m_i}))
% \end{equation}
% is the empirical risk term composed of hinge loss.
% \begin{equation}
% \label{eq:optim3}
%     \min_{W,\b}  \sum_i \|\w_{y_i,m_i}\|^2 \|\phi_i\|^2 + \lambda \sum_i \max (0, 1- (\w_{y_i,m_i}^T \x_i +b_{y_i,m_i}))
% \end{equation}

 The last issue in implementing the above formulation in DNN is that hinge loss provides inferior results compared to  the cross-entropy. 
 \ignore{
 This was demonstrated over a large set of problems \cite{XX} and in fact, the common practice today is to apply only cross-entropy criterion in DNN solving multi-class problems.  However, this issue can be easily mitigated by replacing the hinge loss in Equation~\ref{eq:optim2} with  cross entropy: 
\begin{equation}
{\cal C}_i = - \log (P_{y_i})
\end{equation}
 where $P_{y_i}$ is the conditional probability of the true label $y_i$ as obtained from the network after the softmax layer.  Similarly to  hinge loss, the cross entropy will promote the correct classification while the regularization term will maximize the margin. 
 }
 While for SVM, hinge loss is commonly used, in DNNs the common practice is to use cross-entropy
 %, i.e. ${\cal C}_i = - \log (P_{y_i})$, 
$$
{\cal C}_i = - \log (P_{y_i})
$$
 where $P_{y_i}$ is the probability of the true label $y_i$ obtained from the network after the softmax layer: 
 $$
 P_{y_i}=\frac{e^{s_{y_i}(\x_i)}}{\sum_j e^{s_j(\x_i)} }
 $$
 Similarly to hinge loss, cross-entropy will strive for correct classification while the regularization term will maximize the margin. For the rest of this paper we denote ${\cal R}_i$ as the {\it multi-margin megularization} (MMR).
 
 Note that the regularization term in this scheme is different from the weight decay commonly applied in deep networks. First, here, the minimization is applied over the $\w$ differences of:  $\|\w_{y_i,m_i}\|^2=\|\w_{y_i} -\w_{m_i}\|^2$. Additionally, the regularization term is multiplied by the $\|\phi_{max}\|$.
 Lastly, the regularization term is implemented only at the last layer. 
 %and it does not applied to each layer independently.  

==> 4_selective_sampling.tex <==
\section{Accelerating Training Using Minimal Margin Score Selection}
\label{sec:SelectSample}

\iffalse {The traditional active learning schemes are based on querying labels from a limited budget in an informative and adaptive manner. In a wide range of cases, these schemes offer an exponential reduction in label complexity and therefore an exponential reduction in computation. In more complex and non-convex models such as CNNs, we cannot make any assumptions with respect to the entire model hypothesis space, thus we will direct our focus on the part were the data become more and more linearly separable due to the optimization process, namely, the last fully-connected layer which is also the final classification layer.

We further leverage these concepts and apply our selection based on the samples that are close to the margin in the multi-class scenario. 
}
\fi
\iffalse {
As mentioned above, our method is based on the evaluation of the minimal amount of displacement a training sample should undergo until its predicted classification is switched. We call this measure {\em minimal margin score} (MMS). This measure depends on the best and the 2nd best scores achieved per sample. 
Our measure was inspired by the margin-based quantity suggested by ~\cite{jiang2019predicting} for predicting the generalization gap of a given network. However, in our scheme, we apply our measure to the output layer, and we calculate it linearly with respect to the input of the last layer. Additionally, unlike ~\cite{jiang2019predicting}, we do not take into consideration the true label, and our measure is calculated based on the best and the 2nd best NN scores. }
\fi


We continue to leverage the principle of large margin in neural networks to address the computational limitations in real-world applications, specifically in the selective sampling scheme. We show that by selecting samples that are closer to the margin in the multi-class setting during the forward pass, we achieve better convergence and speed-up during the training process.
To this end, we evaluate our suggested method on CIFAR10 and CIFAR100 using ResNet-44 \cite{he2016deep} and WRN-28-10 \cite{zagoruyko2016wide} architectures. To demonstrate the effectiveness of our selection more vigorously, we apply a faster learning-rate (LR) regime than those suggested in the original papers. 

In principle, our selection method is based on the evaluation of the minimal amount of displacement a training sample should undergo until its predicted classification is switched. We call this measure the {\em minimal margin score} (MMS). This measure depends on the highest and the second highest scores achieved per sample. 
Similarly to our margin-based regularization, we apply our measure only to the output layer, and calculate it linearly with respect to the input of the last layer. Additionally, unlike ~\cite{jiang2019predicting}, we do not take into consideration the true label, i.e., our measure is calculated based solely on the highest and the second highest neural network scores.

As shown in Figure~\ref{fig:mms_new}, a multi-class classification problem is composed of three classes, Green, Red, and Blue, along with three linear projections, $\w_1, \w_2,$ and $\w_3$, respectively. The query point is marked by an empty black circle. The highest scores of the query point are $s^1$ and $s^2$ (assuming all biases are 0's), where $s^1>s^2$ and $s^3$ are negative (not marked). Since the two highest scores are for the Green and Red classes, the distance of the query point to the decision boundary between these two classes is $d$. The magnitude of $d$ is the MMS of this query point.

\ignore{
\begin{figure}[!bht]
% \vspace{-1em}
    \centering
    \includegraphics[width=5cm, height=5cm]{Figures/mms.png}
    \caption{Illustrative example of the MMS measure. }
    \label{fig:mms}
\end{figure}
}


Formally, let $\mathcal{X} = \{\x_1,...,\x_{m}\}$ be a large set of samples and $\phi_i=F(\x_i; \theta) \in \Phi$ be the input to the last layer of the neural network. 
 Assume we have a classification problem with $n$ classes. At the last layer, the classifier $s$ consists of $n$ linear functions: $s_j: \mathcal{\phi} \rightarrow \mathbb{R}$ for $j=1\dots n$ where $s_j$ is a linear mapping $s_j(\phi)=\w_j^T \phi + b_j$.
Denote the sorted scores of $\{s_j(\phi_k)\}_{j=1}^n$ by ${\cal S}=(s_k^{j_1},s_k^{j_2},\cdots,s_k^{j_n})$, where $s_k^{j_p} \geq s_k^{j_{p+1}}$ and  $s_k^{j_p}=s_{j_p}(\phi_k)$.
The classifier $s_{j_1}(\phi_k)$ gives the highest score and $s_{j_2}(\phi_k)$, the second highest score. The {\em decision boundary} between classes $j_1$ and $j_2$ is defined as: 
$$\ell_{12}=\{\phi ~|~ s_{j_1}(\phi)=s_{j_2}(\phi) \}$$
Using this definition, the confidence of the predicted label $j_1$ of point $\phi_k$ is determined  by the distance $d_k$ of $\phi_k$ to the decision boundary $\ell_{12}$.
Following Equation~\ref{eq:d3}, it is easy to show  that
$$
d_k = \frac{s_k^{j_1} -s_k^{j_2} }{\|\w_{j_1} - \w_{j_2}\|}
$$
The distance $d_k$ is the MMS of point $\x_k$. The larger $d_k$, the more confident we are about the predicted label. Conversely, the smaller $d_k$, the less confident we are about the predicted label $j_1$. Therefore, $d_k$ can serve as a confidence measure for the predicted labels. Accordingly, the best points to select for the back-propagation step are the points whose MMS are the smallest. Note that in contrast to the MMR, in this case we do not have to normalize the distance $d_k$ with $\| \phi_{max} \|$ because this normalization will not change the order of ${\cal S}$,
%and the point selection will remain unchanged. 
and thus the set of selected points will remain unchanged.

\iffalse 
{We further leverage these concepts and apply our selection based on the samples that reside in the middle of two candidate classifiers in the multi-class problem. Formally, let $\{x_1,...,x_{B}\} \in \mathbb{D}$ be a large set of samples and $F(\cdot; \theta)$ be the neural network model. Our goal is to select the samples that reduce the volume of the version space induced by the fully-connected classifiers. We claim that this can be achieved by choosing the samples whose confidence level is the minimal. We then introduce a new measure quantity "Maximal Prediction Ratio" (MPR) which will be used as the selection criteria in our scheme.

\begin{align*}
    MPR=\left|\frac{S_{max1} + 1}{S_{max2} + 1}\right|
\end{align*}
where
\begin{align*}
    S_{max1}, S_{max2} = \max_{1 \leq i \leq 2}{F({x_0,..,x_i,...,x_B}, \theta)}\ \ \text{and} \ \ \
    S_{max1} \geq S_{max2}
\end{align*}

We denote $S_{max1}$ and $S_{max2}$ as the predictions scores belonging to the first and second maximal class predictions obtained by the forward pass of the neural network up to and including the fully-connected layer. \enote{Need to explain why this measure will halve the version space and why is it a measure of uncertainty/confidence?} In order to tend the case where both $S_{max1}$ and $S_{max2}$ are very small and negative numbers, we add 1 to each. 
}
\fi
\iffalse
{Our implementation consists of a generic but yet simple online selective sampling method as a preliminary part of the training optimization step. Specifically, at each training step, a selective batch of size $b$ is produced out of a 10 times larger batch before being used in the SGD optimization routine. At a specific iteration, we first apply a forward pass on a batch of size $B$, producing the prediction scores. We then select $b$ samples ($b \ll B$) whose MMS measures are the smallest. This procedure is summarized in Algorithm \ref{alg:batch_select}. 

\begin{figure}
\centering
\begin{minipage}{\textwidth}
\begin{algorithm}[H]
% \noindent
\renewcommand\footnoterule{}
\begin{algorithmic}
\REQUIRE 
Inputs $\mathcal{X}=\{\x_i\}_{i=1}^B$ ,\ $F(\cdot; \theta_0)$ \\%- Training model, b - batch size\\
\STATE{$t \gets 1$}
\REPEAT
\STATE{$\mathcal{Y} \gets F(\mathcal{X}; \theta_{t-1})$ \qquad  \qquad \qquad forward pass on a batch of size B}
\STATE{$MMS \gets d(\mathcal{Y})$ \qquad \qquad \qquad \ \ calculates the Minimal Margin Scores of $\mathcal{Y}$}
\STATE $S \gets \mbox{sort\_index}(MMS,b)$  \  \qquad stores the index of the $b$ smallest scores
\STATE{$\mathcal {X}_b = \{\x_i | ~ i \in \mathcal{S}\}$ \qquad \qquad \qquad subset of $\mathcal{X}$ of size b}
\STATE{$\theta_t \gets sgd\_step(F( \mathcal{X}_b; \theta_{t-1}))$ \qquad back prop. with a batch of size b}
\STATE {$t \gets t+1$} 
\UNTIL{reaching final model accuracy}
\end{algorithmic}
\caption{Selection by Minimal Margin Scores}
\label{alg:batch_select}
\end{algorithm}
\end{minipage}
\end{figure}
}
\fi


Our implementation consists of a generic, yet simple, online selective sampling method, 
%applied as a preliminary part of each training step. 
applied at the beginning of each training step.
Specifically, at each training step, we first apply a forward pass on a batch of points of size $B$, and obtain their respective scores.We then calculate their respective MMS measures, and select the $b$ samples ($b \ll B$) whose MMS measures are the smallest. The resulting batch of size $b$, in turn, is used for training the network. The selection process is repeated every training step, thus potentially selecting a new batch of points for training. The MMS-based training procedure is summarized in Algorithm \ref{alg:batch_select}.

\begin{center}% Or use a figure environment and \centering
\begin{minipage}{1.0\linewidth}
\begin{algorithm}[H]
% \noindent\begin{minipage}{\textwidth}
\renewcommand\footnoterule{}
\begin{algorithmic}[1]
\REQUIRE 
Inputs $\mathcal{X}=\{\x_i\}_{i=1}^B$ ,\ $F(\cdot; \theta_0)$ \\%- Training model, b - batch size\\
\STATE{$t \gets 1$}
\REPEAT
\STATE{${\Phi} \gets F(\mathcal{X}; \theta_{t-1})$ \quad forward pass a batch of size B}
\STATE $MMS \gets d(\Phi)$ \qquad \qquad  \ \ \ \ \ \ \ calc. MMS 
\STATE ${ S} \gets \mbox{sort\_index}(MMS,b)$  \ \ \ \ \ \ store $b$ smallest scores
\STATE{$\mathcal {X}_b = \{\x_i | ~ i \in \mathcal{S}\}$ \qquad \qquad \ \ \ \ subset of $\mathcal{X}$ of size b}
\STATE{$\theta_t \gets sgd\_step(F( \mathcal{X}_b; \theta_{t-1}))$ \ \ back prop. batch of size b}
\STATE {$t \gets t+1$} 
\UNTIL{reaching final model accuracy}
\end{algorithmic}
\caption{MMS-based training}
\label{alg:batch_select}
% \end{minipage}
\end{algorithm}
\end{minipage}
\end{center}

